Crocoddyl: An Efficient and Versatile Framework for Multi-Contact Optimal Control

We introduce Crocoddyl (Contact RObot COntrol by Differential DYnamic Library), an open-source framework tailored for efficient multi-contact optimal control. Crocoddyl efficiently computes the state trajectory and the control policy for a given predefined sequence of contacts. Its efficiency is due to the use of sparse analytical derivatives, exploitation of the problem structure, and data sharing. It employs differential geometry to properly describe the state of any geometrical system, e.g. floating-base systems. Additionally, we propose a novel optimal control algorithm called Feasibility-driven Differential Dynamic Programming (FDDP). Our method does not add extra decision variables which often increases the computation time per iteration due to factorization. FDDP shows a greater globalization strategy compared to classical Differential Dynamic Programming (DDP) algorithms. Concretely, we propose two modifications to the classical DDP algorithm. First, the backward pass accepts infeasible state-control trajectories. Second, the rollout keeps the gaps open during the early "exploratory" iterations (as expected in multiple-shooting methods with only equality constraints). We showcase the performance of our framework using different tasks. With our method, we can compute highly-dynamic maneuvers (e.g. jumping, front-flip) within few milliseconds.

==> src/acknowledgement.tex <==
\section*{Acknowledgment}
\thanks{This research was supported by the European Commision under the Horizon 2020 project Memory of Motion (MEMMO, project ID: 780684).
The authors would also like to thank all the developers of Pinocchio and Eigen which make this work possible by providing high-quality and open-source software.
Last but not least, the authors especially thank Gabriele Buondonno, Joseph Mirabel, Andrea Del Prete, and other members of the MEMMO project for their precious feedback.}


==> src/append.tex <==
\appendix{Derivation of the \gls{ddp} algorithm}
where $\delta\mathbf{x}=\mathbf{\bar{x}} \ominus \mathbf{x}$ is the deviation with respect to the local linearization $\mathbf{\bar{x}}$ and belongs to the tangential space $(\in T_{\mathbf{x}} X)$, and the Jacobian and Hessian of the Hamiltonian are defined as:
\begin{eqnarray}\label{lastQeq}\nonumber
	\mathbf{q}_{\mathbf{x}_k} & = & \mathbf{l}_{\mathbf{x}_k} + \mathbf{f}^T_{\mathbf{x}_k} V_{\mathbf{x}_{k+1}}, \\\nonumber
	\mathbf{q}_{\mathbf{u}_k} & = & \mathbf{l}_{\mathbf{u}_k} + \mathbf{f}^T_{\mathbf{u}_k} V_{\mathbf{x}_{k+1}}, \\
	\mathbf{q}_{\mathbf{xx}_k} & = & \mathbf{l}_{\mathbf{xx}_k} + 
	\mathbf{f}^T_{\mathbf{x}_k} V_{\mathbf{xx}_{k+1}} \mathbf{f}_{\mathbf{x}_k},\\\nonumber
	\mathbf{q}_{\mathbf{xu}_k} & = & \mathbf{l}_{\mathbf{xu}_k} + 
	\mathbf{f}^T_{\mathbf{x}_k} V_{\mathbf{xx}_{k+1}} \mathbf{f}_{\mathbf{u}_k},\\\nonumber
	\mathbf{q}_{\mathbf{uu}_k} & = & \mathbf{l}_{\mathbf{uu}_k} + 
	\mathbf{f}^T_{\mathbf{u}_k} V_{\mathbf{xx}_{k+1}} \mathbf{f}_{\mathbf{u}_k}.
\end{eqnarray}
We obtain the local policy by solving the \gls{qp} \eref{eq:Qeq} as:
\begin{equation}
 \delta\mathbf{u}_k^*(\delta\mathbf{x}_k) = \mathbf{k}_k + \mathbf{K}_k \delta\mathbf{x}_k
\end{equation}
where $\mathbf{k}_k = -\mathbf{q}_{\mathbf{uu}_k}^{-1}\mathbf{q}_{\mathbf{u}_k}$ and $\mathbf{K}_k = -\mathbf{q}_{\mathbf{uu}_k}^{-1}\mathbf{q}_{\mathbf{ux}_k}\delta\mathbf{x}$ are the feedforward and feedback terms, respectively.
And for the next node, we update the quadratic approximation of the value function by injecting $\delta\mathbf{u}^*_k$ expression into \eref{eq:Qeq}:
\begin{eqnarray}\nonumber
 \Delta V(i) &=& -\frac{1}{2}\mathbf{q}_{\mathbf{u}_k} \mathbf{q}_{\mathbf{uu}_k}^{-1}\mathbf{q}_{\mathbf{u}_k} \label{firsteqV}\\
 V_{\mathbf{x}_k} &=& \mathbf{q}_{\mathbf{x}_k} - \mathbf{q}_{\mathbf{u}_k} \mathbf{q}_{\mathbf{uu}_k}^{-1}\mathbf{q}_{\mathbf{ux}_k} \\\nonumber
 V_{\mathbf{xx}_k} &=& \mathbf{q}_{\mathbf{xx}_k} - \mathbf{q}_{\mathbf{ux}_k} \mathbf{q}_{\mathbf{uu}_k}^{-1}\mathbf{q}_{\mathbf{ux}_k} \label{lasteqV}
 \label{lastbackward}
\end{eqnarray}

This backward pass allows us to compute the search direction during the numerical optimization.
Then \gls{ddp} runs a nonlinear rollout (also known as forward pass) of the dynamics to try the computed direction along a step length $\alpha$, i.e.
\begin{eqnarray}\nonumber
 \mathbf{\hat{x}}_0 &=& \mathbf{\tilde{x}}_0 \\
 \mathbf{\hat{u}}_k &=& \mathbf{u}_k + \alpha\mathbf{k}_k + \mathbf{K}_k(\hat{\mathbf{x}}_k \ominus \mathbf{x}_k) \\\nonumber
 \mathbf{\hat{x}}_{k+1} &=& \mathbf{f}_k(\mathbf{\hat{x}}_k,\mathbf{\hat{u}}_k)
\end{eqnarray}
in which we perform a typical \textit{backtracking} line-search by trying first the full step ($\alpha=1$).
Note that $\ominus$ is the \emph{difference} operator between two point that lies in the state manifold.

The \gls{ddp} solver iterates on these two phases -- backward and forward passes -- until convergence to the result (gradient approximately equals zero).



%%%%%%%%%%%% RESULTS
In this section, we first evaluate the performance of \acrshort{crocoddyl} over two design patterns and three different robot models.
For all the cases, we measure the computation time required to solve one iteration.
We use three different robots -- a 7-DoF arm, a quadruped, and a biped -- for analysing our efficient implementation of multi-contact optimal control through holonomic constraints.
Finally, we show that our \gls{fddp} solver can generate highly-dynamic maneuvers in order of milliseconds.
Such kind of motions are hard to generate with classical \gls{ddp} algorithm.

\subsection{CRTP vs VIRT design patterns}
CRTP stands for curiously recurring template pattern.
With this design pattern, the action models are implemented using \emph{static polymorphism} by using variant containers.
It is highly based on standard template meta-programming techniques.
On the other hand, VIRT stands for virtualization designs.
With this design pattern, the action models are defined by \emph{runtime polymorphism} with vector containers.

For comparing the computational performance of CRTP against VIRT design, we solve the LQR problem for different dimensions with 200 nodes using a Intel(R) Core(TM) i5-3210M CPU @ 2.50GHz core frequency.
\fref{fig:crtp_vs_virtual} shows the computation time against LQR dimension for three different cases: 1) CRTP: fixed dimensions of matrices and vectors for the action model and solver, 2) CRTP dyn: only fixed dimensions of matrices and vectors of the solver, and 3) VIRT: dynamic dimensions of any matrix and vector.
As shown in the graphic, CRTP design is faster for all the LQR dimensions, but its benefit dramatically decreases for problem with dimensions typically found in robots with legs and arms.

\begin{figure}[htb]
    \centering
    \includegraphics[width=0.5\textwidth]{figs/crtp_vs_virt-v2.pdf}
    \caption{Computation time against different LQR problem with 200 nodes using a Intel(R) Core(TM) i5-3210M CPU @ 2.50GHz PC.
    The different cases are: 1) CRTP: fixed dimensions of matrices and vectors for the action model and solver, 2) CRTP dyn: only fixed dimensions of matrices and vectors of the solver, and 3) VIRT: dynamic dimensions of any matrix and vector}
    \label{fig:crtp_vs_virtual}
\end{figure}

We have also noticed that with new processors there is no measurable difference between the two polymorphism design patterns.
The main reason here is that AVX instruction sets on modern processors are very efficient for both fixed and dynamic matrices.
These instructions are common in new generation of processors.
As developing with VIRT instead of CRTP polymorphism is much more common, it is easier for new developers to join the project and contribute. It also allows for quicker iteration, debugging, and development. As such, we have taken the decision to follow the virtual polymorphism concept in \gls{crocoddyl}.

\subsection{Different robot models}
Preliminary results indicate computation times reasonable for model predictive control on legged robots.
Computation frequencies are between 50 to 115 Hz for quadruped and biped robots with 60 to 100 nodes.
All these results do not employ parallelization and are the consequence of our efficient method for computing the contact dynamics and its derivatives.


==> src/crocoddyl.tex <==
\section{Crocoddyl Framework}
\acrshort{crocoddyl} has been written in C++ for efficiency and uses the Eigen library for linear algebra routines.
It comes with Python bindings for easy prototyping.
\acrshort{crocoddyl} is currently supported for most Linux distributions, with plans to release on Mac OS X and Windows.
The project is fully open-source under the permissive BSD-3-Clause license and is hosted on GitHub: \url{https://github.com/loco-3d/crocoddyl}.
Compared with~\cite{heried-iros17}, Crocoddyl does not use off-the-shelf solvers such as IPOPT and SNOPT, it exploits the intrisic sparse structure of \gls{ddp}-like solvers.
In the rest of this section, we introduce the main features of \acrshort{crocoddyl}.

\subsection{Analytical and sparse derivatives}
\acrshort{crocoddyl} uses Pinocchio to efficiently compute analytical and sparse derivatives~\cite{carpentier-rss18}.
Pinocchio has dedicated algorithms to compute analytical derivatives of rigid-body algorithms (e.g. \gls{rnea} and \gls{aba}) using spatial algebra \cite{carpentier-rss18}.
\acrshort{crocoddyl} employs these routines to derive the analytical derivative of contact dynamics as described in~\sref{sec:holonomic_ocp}, as well as the ones of cost functions, e.g., \gls{com} tracking, frame placement tracking, etc.
\acrshort{crocoddyl} shares the computation load required for the dynamics, costs, and constraints by storing the data in a common container.

\subsection{Model and data}
One of the main design concepts of \acrshort{crocoddyl} is the strict separation between \textit{model} and \textit{data}.
A \textit{model} describes a system or procedure, e.g. \textit{action}, \textit{cost}, and \textit{activation} models.
Any \textit{model} has been abstracted to easily derive new systems in both C++ and Python.
By \textit{data}, we refer to a container that stores computed and intermediate values used during the calculation routine performed by a \textit{model}.
Each model creates its own data, and with this, we avoid any temporary memory allocation produced by algebraic expressions in Eigen.
To improve efficiency, especially in systems with dimensions lower than 16, the Eigen members inside a data object can be defined with fixed dimensions. It allows for efficient use of modern CPU features by using vectorization and \gls{simd} operations.

\subsubsection{Action models}
The most important model is the \textit{action} one.
An action model combines dynamics, cost, and constraint models.
Each node, in our \gls{oc} problem, is described through an action model.
With this plain description, we can easily model hybrid optimal control problems (or logic-based problem formulations) that typically arise in robots with legs and arms.

To numerically solve the nonlinear \gls{oc} problem, we have to compute a search direction and a step length.
The former procedure is typically computed from the derivatives of the action models --- Jacobians and Hessians.
The latter requires to rollout the dynamics, cost, and constraints along different step lengths.
We have divided both procedures into two main functions: \texttt{calcDiff} and \texttt{calc}, respectively.
The results of these functions (i.e., Jacobians, Hessians, next state, cost value, etc.) are stored inside their corresponding \textit{action data}.
The fact that the memory required for a data object is only allocated once, at the start-up/initialization phase, enhances the time-predictability and parallelizability of the code.
Finally, some of our action models use Pinocchio to efficiently compute rigid-body algorithms and their analytical derivatives~\cite{carpentier-rss18}.
We could easily use numerical and automatic differentiation routines for debugging and prototyping of action models.

\subsubsection{Differential and integrated action models}
It is often convenient to implement action models in continuous time, which we call it \textit{differential action model}.
Together with a predefined \textit{integrated action models}, it is possible to retrieve the time-discrete action model.
Our integrated action models (i.e. integration schemes) conserve the geometrical properties of the system, e.g., the properties of the $\mathbb{SE}(3)$ manifold in a floating-base system.

\subsection{Dealing with geometrical systems}
Generally speaking, the state of the system lies in a manifold $\mathbf{x}\in X$ where its rate of change lies in the tangent space $T_{\mathbf{x}} X$ (see \sref{sec:multibody_ocp}).
% # NB: In the above footnote, we ues Q for a generic manifold
Each manifold obeys to its own algebra, i.e., there are specific rules for the following operations: 
\begin{eqnarray}\label{eq:manifold_operators}
    \mathbf{x}' &=& \mathbf{x} \oplus \delta\mathbf{x}, \nonumber\\
    \delta\mathbf{x} &=& \mathbf{x}_1 \ominus \mathbf{x}_0,
\end{eqnarray}
where $\mathbf{x}\in X$ and $\delta\mathbf{x}\in T_{\mathbf{x}} X$ and can be described by a $n_x$- and $n_{dx}$-tuples, respectively.
These operations are encoded by \texttt{integrate} and \texttt{difference}, respectively.
We also need to define the Jacobians of these operators which are needed for our optimal control solver, i.e.
\begin{eqnarray}\label{eq:manifold_jacobians}
    \hspace{-1em}\frac{\partial\mathbf{x}\oplus\delta\mathbf{x}}{\partial\mathbf{x}}, \frac{\partial\mathbf{x}\oplus\delta\mathbf{x}}{\partial\delta\mathbf{x}} &=& \texttt{Jintegrate}(\mathbf{x},\delta\mathbf{x}), \nonumber\\
    \hspace{-1em}\frac{\partial\mathbf{x}_1\ominus\mathbf{x}_0}{\partial\mathbf{x}_0}, \frac{\partial\mathbf{x}_1\ominus\mathbf{x}_0}{\partial\mathbf{x}_1} &=& \texttt{Jdifference}(\mathbf{x}_0, \mathbf{x}_1),
\end{eqnarray}
where they return the Jacobians for the first and second arguments of the method.
In addition, we have developed efficient and dedicated routines for computing these operations and Jacobians given the URDF model of a multibody system.
Note that for systems that lie in the Euclidean space, these operations are described using linear algebra and Jacobians are the identity matrix.

